Towards Practical Large-scale Randomized Iterative Least Squares Solvers through Uncertainty Quantification

As the scale of problems and data used for experimental design, signal processing and data assimilation grow, the oft-occuring least squares subproblems are correspondingly growing in size. As the scale of these least squares problems creates prohibitive memory movement costs for the usual incremental QR and Krylov-based algorithms, randomized least squares problems are garnering more attention. However, these randomized least squares solvers are difficult to integrate application algorithms as their uncertainty limits practical tracking of algorithmic progress and reliable stopping. Accordingly, in this work, we develop theoretically-rigorous, practical tools for quantifying the uncertainty of an important class of iterative randomized least squares algorithms, which we then use to track algorithmic progress and create a stopping condition. We demonstrate the effectiveness of our algorithm by solving a 0.78 TB least squares subproblem from the inner loop of incremental 4D-Var using only 195 MB of memory.

==> plots/ci_table_noeta.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Tue Apr 26 13:45:46 2022
\begin{longtable}{lrlrrlllll}
  \hline
Sampling Method & Width & Matrix Type & Rows & eta & $>10$ & $>1e-5$ & $>1e-10$ & $>0$ & Total \\ 
  \hline
Achlio & 100 & baart & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}2e-04 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}2e-04 \\ 
  Achlio & 100 & cauchy & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & chebspec & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & chow & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & circul & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & deriv2 & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & dingdong & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & fiedler & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & foxgood & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & frank & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & gilbert & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & golub & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & gravity & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & grcar & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & hadamard & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & hankel & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & heat & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & hilb & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & kahan & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & kms & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & lehmer & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}1e-04 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}1e-04 \\ 
  Achlio & 100 & lotkin & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & magic & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & minij & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & moler & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & oscillate & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & parter & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & pei & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & phillips & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & prolate & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & randcorr & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & rando & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & randsvd & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & rohess & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & rosser & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & sampling & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & shaw & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & smallworld & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & spikes & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & toeplitz & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & tridiag & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & triw & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & ursell & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}2e-04 & \cellcolor{white}0 & \cellcolor{white}2e-04 \\ 
  Achlio & 100 & wilkinson & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & baart & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & cauchy & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & chebspec & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & chow & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & circul & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & deriv2 & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & dingdong & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & fiedler & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & foxgood & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & frank & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & gilbert & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & golub & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & gravity & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & grcar & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & hadamard & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & hankel & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & heat & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & hilb & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & kahan & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & kms & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & lehmer & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & lotkin & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & magic & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & minij & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & moler & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & oscillate & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & parter & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & pei & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & phillips & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & prolate & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & randcorr & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & rando & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & randsvd & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & rohess & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & rosser & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & sampling & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & shaw & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & smallworld & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & spikes & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & toeplitz & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & tridiag & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & triw & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & ursell & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & wilkinson & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & baart & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & cauchy & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & chebspec & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & chow & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & circul & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & deriv2 & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & dingdong & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & fiedler & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & foxgood & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & frank & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & gilbert & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & golub & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & gravity & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & grcar & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & hadamard & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & hankel & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & heat & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}5e-04 & \cellcolor{white}0 & \cellcolor{white}5e-04 \\ 
  gauss & 100 & hilb & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & kahan & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}1e-04 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}1e-04 \\ 
  gauss & 100 & kms & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & lehmer & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & lotkin & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & magic & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & minij & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & moler & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & oscillate & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & parter & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & pei & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & phillips & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}3e-04 & \cellcolor{white}0 & \cellcolor{white}3e-04 \\ 
  gauss & 100 & prolate & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & randcorr & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & rando & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & randsvd & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & rohess & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & rosser & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & sampling & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & shaw & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & smallworld & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & spikes & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & toeplitz & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & tridiag & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & triw & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & ursell & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & wilkinson & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
   \hline
\hline
\end{longtable}


==> plots/eta_tab.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Tue May 17 15:17:54 2022
\begin{longtable}{llrrr}
  \hline
Width & Percent Sampled & Achlio & FJLT & gauss \\ 
  \hline
15 & 0.04 & 5 & 82 & 5 \\ 
  15 & 0.1 & 6 & 91 & 6 \\ 
  15 & 0.39 & 9 & 134 & 9 \\ 
  30 & 0.04 & 6 & 101 & 6 \\ 
  30 & 0.1 & 7 & 106 & 7 \\ 
  30 & 0.39 & 10 & 153 & 11 \\ 
  100 & 0.04 & 9 & 129 & 8 \\ 
  100 & 0.1 & 9 & 141 & 9 \\ 
  100 & 0.39 & 12 & 178 & 14 \\ 
   \hline
\hline
\end{longtable}


==> plots/intervalploterror.tex <==
\begin{tikzpicture}
    \pgfplotsset{
        tmhplot/.style={color=red,opacity = .5,mark=none,line width=6pt,<->},
        omhplot/.style={color=blue,opacity = .5, mark=none,line width=6pt,<->},
        soldot/.style={color=red,only marks,mark=*},
        holdot/.style={color=red,fill=white,only marks,mark=*},
    }
        \begin{axis}[
                xmode = log,
                %width = .9\textwidth,
                %height = .25 \textheight,
                yticklabel style={rotate = 50, anchor = east},
                scaled y ticks=false,
                xmin=0,xmax=3,
                ymin=790,ymax=1010,
                legend pos = south east,
                ytick = {850,900,950,1000},
                %,1050,1100,1150
                yticklabels = {$800-850$,$850-900$,$900-950$,$950-1000$},
                %$1000-1050$,$1050-1100$,$1100-1150$
                ylabel = {Bins for Absolute Error $(\|x_k - x^*\|_2^2)$},
                ylabel style = {anchor = near ticklabel},
                xlabel = {Norm Squared of Gradient},
                title = {$90\%$ Intervals of Gradients Values at Different Error Ranges}
            ]
            %\addplot[omhplot,-,domain=2.24:2.24]{1050};
            
            %\addplot[tmhplot,-,domain=2.09:2.09]{1050};
            
            
            %\addplot[omhplot,-,domain=37.6:37.6]{1150};
            %\addplot[tmhplot,-,domain=32.6:32.6]{1150};
            
            \addplot[omhplot,-,domain=.00245:.0150]{850};
            \addlegendentry{Sketch Grad};
            \addplot[tmhplot,-,domain=.00348:.0132]{850};
            \addlegendentry{True Grad};
            
            \addplot[omhplot,-,domain=.0129:.0771]{900};
            \addplot[tmhplot,-,domain=.0164:.0752]{900};
            
            \addplot[omhplot,-,domain=.0838:.420]{950};
            \addplot[tmhplot,-,domain=.0974:.286]{950};
            
            \addplot[omhplot,-,domain=.446:1.03]{1000};
            \addplot[tmhplot,-,domain=.458:.817]{1000};
            
            %\addplot[omhplot,-,domain=973:1114]{.007};
            %\addplot[tmhplot,-,domain=1011:1120]{.007};
            
        \end{axis}

==> plots/plots/ci_table_noeta.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Tue Apr 26 13:45:46 2022
\begin{longtable}{lrlrrlllll}
  \hline
Sampling Method & Width & Matrix Type & Rows & eta & $>10$ & $>1e-5$ & $>1e-10$ & $>0$ & Total \\ 
  \hline
Achlio & 100 & baart & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}2e-04 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}2e-04 \\ 
  Achlio & 100 & cauchy & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & chebspec & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & chow & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & circul & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & deriv2 & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & dingdong & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & fiedler & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & foxgood & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & frank & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & gilbert & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & golub & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & gravity & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & grcar & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & hadamard & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & hankel & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & heat & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & hilb & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & kahan & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & kms & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & lehmer & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}1e-04 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}1e-04 \\ 
  Achlio & 100 & lotkin & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & magic & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & minij & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & moler & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & oscillate & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & parter & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & pei & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & phillips & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & prolate & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & randcorr & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & rando & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & randsvd & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & rohess & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & rosser & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & sampling & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & shaw & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & smallworld & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & spikes & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & toeplitz & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & tridiag & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & triw & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  Achlio & 100 & ursell & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}2e-04 & \cellcolor{white}0 & \cellcolor{white}2e-04 \\ 
  Achlio & 100 & wilkinson & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & baart & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & cauchy & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & chebspec & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & chow & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & circul & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & deriv2 & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & dingdong & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & fiedler & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & foxgood & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & frank & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & gilbert & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & golub & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & gravity & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & grcar & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & hadamard & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & hankel & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & heat & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & hilb & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & kahan & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & kms & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & lehmer & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & lotkin & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & magic & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & minij & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & moler & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & oscillate & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & parter & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & pei & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & phillips & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & prolate & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & randcorr & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & rando & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & randsvd & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & rohess & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & rosser & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & sampling & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & shaw & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & smallworld & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & spikes & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & toeplitz & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & tridiag & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & triw & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & ursell & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  FJLT & 100 & wilkinson & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & baart & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & cauchy & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & chebspec & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & chow & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & circul & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & deriv2 & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & dingdong & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & fiedler & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & foxgood & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & frank & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & gilbert & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & golub & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & gravity & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & grcar & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & hadamard & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & hankel & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & heat & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}5e-04 & \cellcolor{white}0 & \cellcolor{white}5e-04 \\ 
  gauss & 100 & hilb & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & kahan & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}1e-04 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}1e-04 \\ 
  gauss & 100 & kms & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & lehmer & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & lotkin & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & magic & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & minij & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & moler & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & oscillate & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & parter & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & pei & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & phillips & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}3e-04 & \cellcolor{white}0 & \cellcolor{white}3e-04 \\ 
  gauss & 100 & prolate & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & randcorr & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & rando & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & randsvd & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & rohess & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & rosser & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & sampling & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & shaw & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & smallworld & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & spikes & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & toeplitz & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & tridiag & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & triw & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & ursell & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
  gauss & 100 & wilkinson & 512 & 1 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 & \cellcolor{white}0 \\ 
   \hline
\hline
\end{longtable}


==> plots/plots/eta_tab.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Tue May 17 15:17:54 2022
\begin{longtable}{llrrr}
  \hline
Width & Percent Sampled & Achlio & FJLT & gauss \\ 
  \hline
15 & 0.04 & 5 & 82 & 5 \\ 
  15 & 0.1 & 6 & 91 & 6 \\ 
  15 & 0.39 & 9 & 134 & 9 \\ 
  30 & 0.04 & 6 & 101 & 6 \\ 
  30 & 0.1 & 7 & 106 & 7 \\ 
  30 & 0.39 & 10 & 153 & 11 \\ 
  100 & 0.04 & 9 & 129 & 8 \\ 
  100 & 0.1 & 9 & 141 & 9 \\ 
  100 & 0.39 & 12 & 178 & 14 \\ 
   \hline
\hline
\end{longtable}


==> plots/plots/intervalploterror.tex <==
\begin{tikzpicture}
    \pgfplotsset{
        tmhplot/.style={color=red,opacity = .5,mark=none,line width=6pt,<->},
        omhplot/.style={color=blue,opacity = .5, mark=none,line width=6pt,<->},
        soldot/.style={color=red,only marks,mark=*},
        holdot/.style={color=red,fill=white,only marks,mark=*},
    }
        \begin{axis}[
                xmode = log,
                %width = .9\textwidth,
                %height = .25 \textheight,
                yticklabel style={rotate = 50, anchor = east},
                scaled y ticks=false,
                xmin=0,xmax=3,
                ymin=790,ymax=1010,
                legend pos = south east,
                ytick = {850,900,950,1000},
                %,1050,1100,1150
                yticklabels = {$800-850$,$850-900$,$900-950$,$950-1000$},
                %$1000-1050$,$1050-1100$,$1100-1150$
                ylabel = {Bins for Absolute Error $(\|x_k - x^*\|_2^2)$},
                ylabel style = {anchor = near ticklabel},
                xlabel = {Norm Squared of Gradient},
                title = {$90\%$ Intervals of Gradients Values at Different Error Ranges}
            ]
            %\addplot[omhplot,-,domain=2.24:2.24]{1050};
            
            %\addplot[tmhplot,-,domain=2.09:2.09]{1050};
            
            
            %\addplot[omhplot,-,domain=37.6:37.6]{1150};
            %\addplot[tmhplot,-,domain=32.6:32.6]{1150};
            
            \addplot[omhplot,-,domain=.00245:.0150]{850};
            \addlegendentry{Sketch Grad};
            \addplot[tmhplot,-,domain=.00348:.0132]{850};
            \addlegendentry{True Grad};
            
            \addplot[omhplot,-,domain=.0129:.0771]{900};
            \addplot[tmhplot,-,domain=.0164:.0752]{900};
            
            \addplot[omhplot,-,domain=.0838:.420]{950};
            \addplot[tmhplot,-,domain=.0974:.286]{950};
            
            \addplot[omhplot,-,domain=.446:1.03]{1000};
            \addplot[tmhplot,-,domain=.458:.817]{1000};
            
            %\addplot[omhplot,-,domain=973:1114]{.007};
            %\addplot[tmhplot,-,domain=1011:1120]{.007};
            
        \end{axis}
